Dependency Practices for Vulnerability Mitigation

Relying on dependency packages accelerates software development, but it also increases the exposure to security vulnerabilities that may be present in dependencies. While developers have full control over which dependency packages (and which version) they use, they have no control over the dependencies of their dependencies. Such transitive dependencies, which often amount to a greater number than direct dependencies, can become infected with vulnerabilities and put software projects at risk. To mitigate this risk, Practitioners need to select dependencies that respond quickly to vulnerabilities to prevent the propagation of vulnerable code to their project. To identify such dependencies, we analyze more than 450 vulnerabilities in the npm ecosystem to understand why dependent packages remain vulnerable. We identify over 200,000 npm packages that are infected through their dependencies and use 9 features to build a prediction model that identifies packages that quickly adopt the vulnerability fix and prevent further propagation of vulnerabilities. We also study the relationship between these features and the response speed of vulnerable packages. We complement our work with a practitioner survey to understand the applicability of our findings. Developers can incorporate our findings into their dependency management practices to mitigate the impact of vulnerabilities from their dependency supply chain.

==> Acknowledgements.tex <==
The authors are grateful to the respondents who dedicated their time to participate in our surveys. The involvement of human participants in this study was approved by Concordia University’s Faculty Research \& Ethics Advisory Committee (summary protocol form number: 30004729).
\color{black}

==> Dependency_Smells.tex <==

In this section, we define each dependency smell, the rationale for why it might occur, and its negative consequences (\Cref{sub:smells-catalog}). \rev{Similar to the code smell literature, whether or not something is a smell is based on the context \cite{fontana2016antipattern}}.
 These smells have not been explicitly defined in the literature. They are initially observed by studying violations of \npm recommendations, violations of SemVer guidelines and by studying the discussions surrounding the package.json file. We have followed up the initial observations with a survey from twelve practitioners in the field to better understand the negative consequences of each smell and why they might occur.
We sent out an open-format questionnaire (where respondents are free to write anything) to seventeen JavaScript developers that we knew had sufficient experience with developing JavaScript projects. \rev{The developers were a convenient sample from Canada and Brazil that were known by the authors. They were contacted by email.} We presented them with different approaches of depending on an \npm package and asked them to write down the advantages and disadvantages associated with each approach. Since we did not want to bias the developers into associating negative consequences with the presented approaches, we refrained from calling an approach a ``smell'' and also included the SemVer-compliant alternative among our approaches. More importantly, we asked them to give us both advantages and disadvantages for each approach. The advantages not only help in reducing bias but also help in understanding why a particular dependency smell might occur. In order to ensure a similar understanding of dependency management and SemVer, we provided the participants with links to the \npm dependency reference \cite{npmpkg2019} and the SemVer standard guide \cite{semver2019} .

From the seventeen invites, twelve developers responded to our first survey (i.e,. 70\% of response rate).
From the 12 respondents, 10 identified themselves as industry practitioners and 2 participants were students.
All participants have used \npm and 11 out of 12 participants had at least one year of experience in Node.JS development. 
From the 12 respondents, 11 were familiar with SemVer.
For each dependency smell, we categorized the 12 responses using an open-coding approach similar to the guidelines expressed by Philip Burnard \cite{burnard1991method}. Through an iterative process for each smell, we extracted and grouped relevant themes from developer responses into reasons for why a smell occurs and reasons for why it can cause problems.

\rev{The smells identified in this paper focus on \textit{how} dependencies are used and managed, rather than \textit{what} dependencies are selected. Therefore, issues such as using too many dependencies or the wrong selection of dependencies are not covered, as they are specific to the requirements and functionalities of each project.}

\subsection{Dependency Smells Catalog}
\label{sub:smells-catalog}

This smells catalog consists of a list of seven identified dependency smells. We do not claim this to be an exhaustive list, but given that \npm limits the possible expressions of dependency constraints in the package.json file, the smells presented here cover the majority of different alternatives for depending on a package. Figure~\ref{fig:packagejson} presents examples of the restrictive constraint, pinned dependency, permissive constraint, and URL dependency smells. Other dependency smells are not identifiable solely by looking at the package.json file and they require closer inspection of the source code or project directory.

In identifying the negative consequences associated with each pattern, along with the reasons for why they might occur, we relied on developers' feedback as well as the inherent \npm rules for evaluating dependency constraints. In each smell's definition, we give examples of developer responses (Tagged P1 through P12). Table~\ref{tab:overview} presents an overview of the smells and their negative consequences.

Note that in this first survey we did not ask about the Unused Dependency and the Missing Dependency smell.
\rev{These smells are included as they are both a clear case of dependency mismanagement. They create a mismatch between dependencies used in the source code and the ones defined in package.json which is a violation of npm guidelines \cite{npmpkg2019}. Hence, we do not expect any developers to consider them as a valid approach with positive outcomes. Missing dependencies can cause runtime errors or crashes when executing the code that relies on the dependency. Unused dependencies unnecessarily increase installation size and maintenance effort required for dependencies. Soto-Valero et al. \cite{soto2020comprehensive} use the term bloated dependencies to study unused dependencies in the Maven ecosystem. Depcheck is an npm tool which reports unused and missing dependencies for npm projects \cite{depcheck2019}.}
Additionally, we did not ask developer’s opinion on not using package lock, which is the smell in our catalog (No package-lock). Instead, we ask the advantages and disadvantages of \textit{using} package.lock in the project, given this more intuitive and easier to assess than the consequences of not using an approach. We then use the pros of using a package.lock as the cons of not having package.lock in the project, and vice versa.
\\
\begin{table*}[t]
	\centering
	\caption{Overview of dependency smells.}
	\label{tab:overview}
	\input{tables/overview}
\end{table*}


%\subsection{Pinned dependency}
\noindent\textbf{\large{S1 - Pinned dependency: }}

\noindent\textbf{Description:}
A pinned dependency is a type of restrictive approach in which only a single version of the dependency is accepted, for example pinning to version 1.2.3.

\noindent\textbf{Why it occurs:}
Choosing to pin dependencies is a common approach to ensure fine-grained control over the software packages that a project depends on. It is sometimes even recommended for runtime dependencies of deployable projects to ensure consistent installations. %, even though it does not guarantee the indirect dependencies will remain at a fixed version.
This approach drastically reduces the risk of breaking changes and unknown bugs or vulnerabilities that may exist only in newer releases. For example, P12 said: \textit{``Makes it extremely unlikely for breaking changes to happen ...''}.

\noindent\textbf{When it is a dependency smell:}
By pinning a dependency, we will not receive important security and bug fixes, as P12 mentions: \textit{``you are more exposed to security risks and bugs"}. It therefore leaves our project less and less secure over time, unless manual measures are taken to constantly update the constraint to a newer version, which will require extra effort. For example, P10 said: \textit{``[It] creates technical debt in dependencies. Someone has to put in the time later to update them ...''}. Having pinned dependencies is even worse for packages which will later be used as dependencies in other projects, since \npm can no longer re-use similar dependencies for installed packages but must rather have separate installations for the different versions, which can cause a significant increase in the number of installed dependencies for a project. For example, P10 cited: \textit{``...increases node modules size because different packages can’t share the same installation''}.
\\

%\subsection{URL dependency}
\noindent\textbf{\large{S2 - URL dependency: }}

\noindent\textbf{Description:}
URL dependencies are constraints that directly point to an online URL, often pointing to a repository link such as GitHub. The URL may point to a general repository or a specific release or branch in that repository. Figure~\ref{fig:packagejson} contains an example of a URL dependency.

\noindent\textbf{Why it occurs:}
The most plausible reason for choosing a URL dependency is in cases where there is no equivalent on the \npm package manager, as P2 states: \textit{``Point to a package outside \npm listings''}. Another potential reason is instances where the dependent strongly needs a new fix in the repository that has not yet made its way to the latest release on \npm. For example, P7 said: \textit{``... the fix is applied to the GH repo way before we see it on \npm. ...''}.

\noindent\textbf{When it is a dependency smell:}
URL dependency constraints are problematic for a variety of reasons. If the URL points to a master branch of a software repository it can lead to breaking changes since any new change to the master branch will be fetched. If the URL points to a specific release of a package on a repository or other type of webpage, it is akin to a pinned dependency. In any case, it is very difficult to adhere to SemVer guidelines whilst using URL constraints for dependencies. In addition, since developers are operating outside \npm, they cannot take advantage of its project metrics and security advisories, and they are more vulnerable to typosquatting attacks (different and malicious packages with very similar names) \cite{npmtypo2017}. Apart from security issues, the unstable nature of unreleased packages can also introduce more bugs, as mentioned by P9: \textit{``... vulnerable to typo-squatting attacks and even if the repository is legit, you are depending on something unstable ...''}. It can also be harder to identify if a new version is released if the URL does not point to a code repository. Additionally, \npm prohibits the deletion of uploaded packages after a grace period, but a URL can change or be removed completely at the owner's discretion, leaving developers with missing dependencies. For example, P8 cites: \textit{``If the linked library disappear then code will stop working ...''}. If the package exists on \npm, one should use the published version. Otherwise, it may be possible to avoid this dependency in favor of its \npm-established alternative.
\\

%\subsection{Restrictive constraint}
\noindent\textbf{\large{S3 - Restrictive constraint: }}

\noindent\textbf{Description:}
Restrictive constraints are any dependency constraints that are more restrictive than SemVer. For post-1.0.0 releases, this is equivalent to only accepting patch updates using the "\textasciitilde" notation (e.g. \textasciitilde2.1.3) or by using the "x" notation in the patch component of a constraint (e.g. 2.1.x).
While pinned dependencies are a special case of restrictive constraint, we opt for separating them in our study for clarity purposes.
%In this study, we separate pinned dependencies from restrictive constraints.

\noindent\textbf{Why it occurs:}
When a developer knowingly opts for a more restrictive approach in specifying dependency constraints, it is likely due to fear of breaking changes from automatic updates. For example, P12 said: \textit{``... reduce[s] the chance of breakage"}. Indeed, adhering to SemVer only guarantees backward compatible updates if the maintainers of the dependency also adhere to SemVer. This verification is not straightforward and it can be difficult to ensure backward compatibility in practice \cite{decan2019}. Nonetheless, restrictive constraints still allow patch updates, as P8 states: \textit{``This will make sure your libraries are up to date in regard to security patches"}.

\noindent\textbf{When it is a dependency smell:}
Restrictive constraints prevent the project from receiving backward compatible updates. For example, P10 mentions: \textit{``I will not get "safe" feature updates"}. In practice however, the situation could be even worse. Since minor releases can also contain crucial fixes which are not necessarily back-ported to previous patch releases, using the restrictive constraint does not even guarantee we will receive the majority of important security or bug fixes. For example, P9 states: \textit{``quite common to see lots of bugs and vulnerabilities addressed in a minor which never make it to any of the previous patch releases"}. Alternatively, restrictive dependencies have to be manually changed more frequently to keep up with newer versions. This creates extra work for developers, as mentioned by P2: \textit{``Increased work required to update the system"}.
\\

%\subsection{Permissive constraint}
\noindent\textbf{\large{S4 - Permissive constraint:}}

\noindent\textbf{Description:}
Permissive constraints are any dependency constraints that are more permissive than SemVer. For post-1.0.0 releases, this is equivalent to accepting major updates using the * or "" wildcards, or by specifying a minimum version range without a maximum limit such as $>1.2.3$.

\noindent\textbf{Why it occurs:}
In cases where there is an inter-dependency between dependencies maintained by the same developers, they might freely accept any updates since they are in charge of both projects and are therefore more confident in the type of changes they make. For some, removing restrictions is an easy way to make sure the latest updates are fetched. For example, P9 said: \textit{``It caters to my inner laziness"}.

\noindent\textbf{When it is a dependency smell:}
Permissive constraints expose projects to the constant risk of breaking changes, as stated by P10: \textit{``Sooner or later, an update will break the API"}. If the maintainers pinpoint the breaking changes immediately, they have to manually change the constraint to an earlier version, which they have first to identify to work correctly. This is not always easy if semantically breaking changes have creeped up during several updates. %Otherwise, users of the project will be unhappy that the project no longer builds or functions correctly.
In addition, it is irrational to claim a project will work with all future versions of a dependency. In fact, the Cargo ecosystem has prohibited the use of wildcards for this very reason \cite{cargowild2018}.
\\

%\subsection{No package-lock}
\noindent\textbf{\large{S5 - No package-lock: }}

\noindent\noindent\textbf{Description:}
The \npm package-lock file includes the entire dependency tree with precise dependency versions at a specific time, which make sure the project will be built. The \npm documentation recommends that the package-lock should be committed into source repositories \cite{npmpkglock2019}. However, we observe that developers do not always include package-lock (or its similar counterparts: yarn.lock or npm-shrinkwrap.json) in their project repositories.

\noindent\textbf{When it occurs:}
Since package-lock is auto-generated, this smell occurs because developers chose not to commit the file into their repository. Since the package-lock does not affect the package.json file and it can be rebuilt if the desired dependencies change, or it can be ignored altogether, we do not see any rationale for not including it, and developers seem to generally agree. For example, P12 said: \textit{``I don't see any issues with having package-lock"}.

\noindent\textbf{Why it is a dependency smell:}
In the absence of the package-lock file, there is no way to guarantee that installation at different times will yield the same result (even if the dependencies are pinned), as stated by P10: \textit{``everyone can use it [package-lock] to install the same exact thing"}. In a sense, package-lock provides the best of both worlds by allowing developers to comfortably use SemVer in their package.json file while giving the option to install using a pinned dependency tree. Without a package-lock there is no way to track the history of dependencies without uploading the large node\_modules folder. For example, P9 mentions: \textit{``... if I don’t use package-lock ... I need to push my node modules folder"}.
\\

\noindent\textbf{\large{S6 - Unused dependency:}}

\noindent\textbf{Description:}
The unused dependency smell represents runtime dependencies that exist in the package.json file, but are not used in source code of the project.

\noindent\textbf{Why it occurs:}
The unused dependency occurs when the code and import statements that needed the dependency were removed but the package.json file has not been cleaned up to properly reflect this. Alternatively, the dependency may only be used in development environments but it is incorrectly listed under runtime dependencies instead of the development dependencies in the package.json file.

\noindent\textbf{When it is a dependency smell:}
If the dependency was actually removed from the project, then including it in the package.json file will cause an extraneous package installation and take up unnecessary space in the modules folder. Even if the dependency is used in development but incorrectly specified under runtime dependencies rather than development dependencies, it will result in the same extraneous installation when installing a project for production. Additionally, both cases will cause confusion for users and developers of the project. In any case, a mismatch between the dependencies imported in the source code and the ones defined in the package.json is a violation of \npm guidelines \cite{npmpkg2019}.
\\

\noindent\textbf{\large{S7 - Missing Dependency: }}

\noindent\textbf{Description:}
The missing dependency smell represents packages that are used in the source code, but not specified in the runtime dependencies of the package.json file.

\noindent\textbf{Why it occurs:}
The missing dependency smell can occur when a dependency is manually installed but not added to the package.json (by using the `--save' option with the \npm install command). Additionally, it can appear because the dependency is removed from the project, and thus the package.json file, but the import statements are not fully cleaned up from the code. Alternatively, a missing dependency may still be used in the code but it has not yet raised errors because it exists in a seldom-reached execution path.

\noindent\textbf{When it is a dependency smell:}
Missing dependencies can be very problematic if they are in fact used in the source code but are not properly specified in the package.json file. This can result in bugs or crashes while executing the part of the source code that relies on this dependency. If the missing dependency occurs because the dependency is imported in source code but never actually used, it will still create ambiguity for users and developers of the source code. In any case, a mismatch between the dependencies imported in the code and the ones defined in the package.json is a violation of \npm guidelines \cite{npmpkg2019}.


\color{black}

\color{blue}




%To that aim, we asked practitioners to rate their level of agreement on a scale of 1 to 5 (strongly disagree, disagree, neither, agree, strongly agree) on each of the statements shown in \Cref{tab:initial_sur}.
%with a wider audience of 41 practitioners to quantify the impact of each dependency smell. In this new survey, we asked practitioners to rate their level of agreement on a scale of 1 to 5 (strongly disagree, disagree, neither, agree, strongly agree) on each of the statements (advantages and disadvantages) extracted from the first survey. %\textcolor{red}{explain here how and why you added missing and unused deps}
%\abbas{should we code statements from a table? or should we have full statements?}

%\begin{figure}[h]
%  \centering
% \includegraphics[width=\linewidth]{figures/chart}
%  \caption{Example of a smelly package.json file}
%  \label{fig:chart}
%  \Description{chart}
%\end{figure}

\color{black}


==> Discussion.tex <==
While our study focuses on \npm, many of these smells can apply to other ecosystems with varying degrees. In fact, any package manager that allows developers to restrict dependencies to a particular version or version range is susceptible to pinned and restrictive dependency smells. It will also be susceptible to permissive and URL dependency smells if the package managers allow developers to always use the latest version of a package or fetch a dependency directly from a URL. Missing dependencies (and to a lesser extent, Unused dependencies) are mainly a problem for interpreted languages such as JavaScript and Python. However, compiled languages such as C++ (and even languages like Java) can catch these issues at compile time.
For example, the PyPI ecosystem for Python allows developers to specify dependencies (requirements specifiers) and constraints (version specifiers) in a setup.py or requirements.txt file. The Python dependency specification \cite{pipsemver} allows for a pinned dependency using the version matching clause (==). PyPI also uses the compatible release clause ($\sim=$) and the ordered comparison clause ($>$= and $<$=) which allows for the restrictive constraint and permissive constraint smells. Python projects can also suffer from unused and missing dependencies since one can specify dependencies regardless of their usage in the code, or forget to specify all dependencies in the setup.py or requirements.txt file. PyPI allows direct URL links using the ``$<$Dep Name$>$ @ $<$URL$>$" format. PyPI also uses the pip-freeze command to output installed package versions which can be used for locking dependencies, similar to package-lock in \npm. \\
\indent{It is worthwhile mentioning that while other ecosystems can differ in the type of smells they can experience, the severity of the smells might also be different. A good example is the difference in the way the JavaScript and Python package managers handle dependency conflicts. While \npm handles conflicts by installing multiple versions of a transitive dependency, which are each nested inside their respective direct dependencies \cite{npminstall}, PyPI will either outright reject installing incompatible Python packages or break another dependency by installing an incompatible transitive dependency \cite{pipguide}. This means that while using pinned dependencies can cause security issues in both ecosystems (due to not receiving security updates), in the case of Python, it can also break dependencies, while for \npm, it will only increase the installation size.}


\color{black}


==> Evolution.tex <==

\begin{figure*}
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\textwidth]{figures/pinned-introduced-fixed.pdf}
    \caption{\small Pinned Dependency}
    \label{pinned-introduced-fixed}
  \end{subfigure}
  %
  \hspace{-1mm}%
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\textwidth]{figures/url-introduced-fixed.pdf}
    \caption{\small URL Dependency}
    \label{url-introduced-fixed}
  \end{subfigure}
%
\hspace{-1mm}%
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\textwidth]{figures/restrictive-introduced-fixed.pdf}
    \caption{\small Restrictive Constraint}
    \label{restrictive-introduced-fixed}
  \end{subfigure}
  %
  \hspace{-1mm}%
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\textwidth]{figures/wildcard-introduced-fixed.pdf}
    \caption{\small Permissive Constraint}
    \label{wildcard-introduced-fixed}
  \end{subfigure}
 %
\caption{Introduced and fixed dependency smells over time.}
\label{fig:smells-introduced-fixed}
\end{figure*}

\begin{figure*}
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{figures/pinned-accumulation.pdf}
		\caption{\small Pinned Dependency}
		\label{pinned-accumulation}
	\end{subfigure}
	%
	  \hspace{-1mm}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{figures/url-accumulation.pdf}
		\caption{\small URL Dependency}
		\label{url-accumulation}
	\end{subfigure}
	%
	  \hspace{-1mm}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{figures/restrictive-accumulation.pdf}
		\caption{\small Restrictive Constraint}
		\label{restrictive-accumulation}
	\end{subfigure}
	%
	  \hspace{-1mm}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{figures/wildcard-accumulation.pdf}
		\caption{\small Permissive Constraint}
		\label{wildcard-accumulation}
	\end{subfigure}
	%
	\caption{Accumulation of dependency smells over time.}
	\label{fig:accumulation}
\end{figure*}

Now that we know dependency smells are prevalent, we want to investigate smell-inducing and smell-fixing commits throughout history to better understand their evolution. By analyzing the smells that were introduced or fixed in the past five years, we can better understand when these smells started to accumulate and where the current trend is moving towards.


Since we have the contextual diff for all commits parsed and stored into our database, we can identify when and how dependency constraints were changed throughout the project. We specifically focused only on dependencies that persist between two commits but their constraint was changed such that a dependency smell was introduced or fixed. This prevents noisy data due to fixes that are merely a result of dependency removal or migration. Since the analyses for this research question rely on the dependency constraints inside the package.json file, it can only be conducted on the first four dependency smells (pinned dependency, URL dependency, restrictive constraint, and permissive constraint). We have analyzed the changes over a 5 year period to provide a more comprehensive view of how the smells evolve through time.

\begin{table}
	\centering
	\caption{Number of introduced and fixed instances per dependency smell.}
	\label{tab:instances}
	\input{tables/introduced-fixed-per-smell}
\end{table}

Table~\ref{tab:instances} presents the total number of instances for each of the four smells that were introduced or fixed during a five-year period from mid 2014 to mid 2019. The line plots in Figure~\ref{fig:smells-introduced-fixed} show how the introduction and fix of dependency smells happen throughout project evolution. The fixed lines clearly show that developers are somewhat aware of these smells and they regularly address them.

In order to investigate whether the regular fixes are enough to alleviate the regular introduction of dependency smells, we have plotted the accumulation of these dependency smells in Figure~\ref{fig:accumulation}. \rev{This accumulation is normalized by the number of projects included in the dataset per month (since projects are added at different times).} As can be seen, the pinned dependency, URL dependency, and restrictive constraint smells have an increasing trend. This shows that despite consistent dependency refactoring throughout the history of these projects, the number of newly added dependency smells are still higher.

The accumulation graph for the permissive constraint smell is noticeably different than the rest, both in its spiky form and its recently downwards trend. The non-gradual shape of the diagram might be due to the smaller number of instances for this smell (Table~\ref{tab:instances}). The permissive constraint smell subjects projects to a higher risk of breaking changes and the recently decreasing trend implies that developers generally agree that this smell is not justified, or the drawbacks far outweigh any benefits. It may be for this reason that another ecosystem like Cargo has banned the use of permissive wildcards in 2016 \cite{cargowild2018}. \rev{It may also be due to the severity of this smell. According to  \Cref{tab:initial_sur}, Permissive Constraints have the highest likelihood of introducing breaking changes. Another reason for this downward trend could be the introduction of the semver-compliant caret (\textsuperscript{$\wedge$}) symbol in \npm and its use as the default in February 2014 \cite{decan2019, nodesource}. This gives developers more freedom by allowing minor and patch updates (as opposed to only patch updates) and discourages the use of more permissive constraints..}

Dependency smells are addressed and fixed through time, but most dependency smells are introduced more frequently than they are fixed, causing an accumulation of smells over time. The permissive constraint smell is the only case where we observed a decrease over time.



==> tables/survey_agreement.tex <==
%\multirow{4}{*}{\shortstack{Restrictive \\Constraint}} 

\newcommand{\colsize}{1.4cm}
\newcommand{\tablequote}[1]{\textit{#1}}
\newcommand{\tablestm}[1]{\textbf{#1}}
\newcommand{\pro}{$+$}
\newcommand{\con}{$-$}
\begin{tabular}{p{2cm}|p{6.5cm}|p{6.5cm}}
		\toprule
		
		
		\multirow{2}{\colsize}{Smell / Approach}  
		& \multirow{2}{*}{Statement}
		& Second qualitative survey results
		
		%\cline{1-2}		
		
		
		&  & \\
		\cmidrule{1-2} 
		\cmidrule{4-4} 

		
		% PINNED DEPENDENCY
		\multirow{8}{\colsize}{Pinned Dependency}  
		  & \tablestm{\con~Increases bugs and vulnerabilities over time}  & 
		    \\  %\cline{2-2}
			& & \\  %\cline{2-2}
		   & \tablestm{\con~Increases installation size} & 
		   \\
			& & \\  %\cline{2-2}
		   & \tablestm{\con~Creates extra overhead for manually updating} & 
		   \\  %\cline{2-2}
		& & \\  %\cline{2-2}
		   & \tablestm{\pro~Drastically reduces breaking changes} & 
		   
		   \\  \cline{4-4}
   		\cmidrule{1-2}
   		%[3ex] %\cline{1-2}
   		
   		% URL DEPENDENCY
   		\multirow{8}{\colsize}{URL Dependency}
		& \tablestm{\con~Can cause dependency breakage (link-removal)}  & 
		\\
		&  &\\  %\cline{2-2}
		  & \tablestm{\con~Increases security risk and bugs}
		  
		  &  \hspace{-0.1cm}
		  \raisebox{-.712\height}[0pt][0pt]{\includegraphics[height=30\normalbaselineskip]{figures/stacked_plot.pdf}} 
		  \\ %[3ex] %\cline{2-2}
		  & \tablestm{\pro~Useful for non-\npm packages and custom forks}  & 
		 		  \\
		  & &\\   %\cline{2-2}
		  & \tablestm{\pro~Useful for getting latest fixes not yet published}   & 
		  		  \\
		  &   &\\ 
		  \cline{4-4}
		   \cmidrule{1-2}
   		
   		
		\bottomrule
	\end{tabular}
